Towards Characterizing International Routing Detours

There are currently no requirements (technical or otherwise) that BGP paths must be contained within national boundaries. Indeed, some paths experience international detours, i.e., originate in one country, cross international boundaries and return to the same country. In most cases these are sensible traffic engineering or peering decisions at ISPs that serve multiple countries. In some cases such detours may be suspicious. Characterizing international detours is useful to a number of players: (a) network engineers trying to diagnose persistent problems, (b) policy makers aiming at adhering to certain national communication policies, (c) entrepreneurs looking for opportunities to deploy new networks, or (d) privacy-conscious states trying to minimize the amount of internal communication traversing different jurisdictions. In this paper we characterize international detours in the Internet during the month of January 2016. To detect detours we sample BGP RIBs every 8 hours from 461 RouteViews and RIPE RIS peers spanning 30 countries. Then geolocate visible ASes by geolocating each BGP prefix announced by each AS, mapping its presence at IXPs and geolocation infrastructure IPs. Finally, analyze each global BGP RIB entry looking for detours. Our analysis shows more than 5K unique BGP prefixes experienced a detour. A few ASes cause most detours and a small fraction of prefixes were affected the most. We observe about 544K detours. Detours either last for a few days or persist the entire month. Out of all the detours, more than 90% were transient detours that lasted for 72 hours or less. We also show different countries experience different characteristics of detours.

==> detour_origin_destination_analysis.tex <==
% !TEX root = main.tex
%Talk about using the ground truth datasets
\subsection{Detour Origin and Destination Analysis}

\comment{
\begin{itemize}
\item{Top Detour Origin}
\item{Top Detour Destination}
\item{Any Malicious ASes from ASWatch?}
\end{itemize}
}




